Robotic Constrained Imitation Learning for the Peg Transfer Task in Fundamentals of Laparoscopic Surgery

In this study, we present an implementation strategy for a robot that performs peg transfer tasks in Fundamentals of Laparoscopic Surgery (FLS) via imitation learning, aimed at the development of an autonomous robot for laparoscopic surgery. Robotic laparoscopic surgery presents two main challenges: (1) the need to manipulate forceps using ports established on the body surface as fulcrums, and (2) difficulty in perceiving depth information when working with a monocular camera that displays its images on a monitor. Especially, regarding issue (2), most prior research has assumed the availability of depth images or models of a target to be operated on. Therefore, in this study, we achieve more accurate imitation learning with only monocular images by extracting motion constraints from one exemplary motion of skilled operators, collecting data based on these constraints, and conducting imitation learning based on the collected data. We implemented an overall system using two Franka Emika Panda Robot Arms and validated its effectiveness.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
% for not arxiv
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
%      colorlinks=true,%
%      linkcolor=black, %%追加20090108
%      citecolor=black, %%追加20090108
%      urlcolor=black, %%追加20090108
%      bookmarksopen=true,%しおりツリーをデフォルトで開く
%      ]{hyperref}
% \usepackage[dvipdfmx]{graphicx}
% for arxiv
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}

\usepackage{url}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}

\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}

\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\tabref}[1]{{Table \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

